DROGON: A Trajectory Prediction Model based on Intention-Conditioned Behavior Reasoning

We propose a Deep RObust Goal-Oriented trajectory prediction Network (DROGON) for accurate vehicle trajectory prediction by considering behavioral intentions of vehicles in traffic scenes. Our main insight is that the behavior (i.e., motion) of drivers can be reasoned from their high level possible goals (i.e., intention) on the road. To succeed in such behavior reasoning, we build a conditional prediction model to forecast goal-oriented trajectories with the following stages: (i) relational inference where we encode relational interactions of vehicles using the perceptual context; (ii) intention estimation to compute the probability distributions of intentional goals based on the inferred relations; and (iii) behavior reasoning where we reason about the behaviors of vehicles as trajectories conditioned on the intentions. To this end, we extend the proposed framework to the pedestrian trajectory prediction task, showing the potential applicability toward general trajectory prediction.

==> dataset.tex <==


% \begin{table}[]
% \begin{center}
% \begin{tabular}{llcccl}
% \hline

%                               &                   & KITTI~\cite{Geiger2012CVPR} & TrafficPredict~\cite{ma2019trafficpredict} & Ours \\ \hline \hline
% No. of scenarios              &                   & 50    & 103                    & \textbf{213}     \\ \hline
% No. of frames ($\times10^3$)                 &                   & 13.1      & \textbf{90}                       & 59.4     \\ \hline %59470
% No. of object classes                &                   & 8     & 5                      & \textbf{8}  \\ \hline 
% No. of intersections          &                   & -     & -                      & \textbf{213}  \\ \hline 
% Sampling frequency (fps)      &                   & 10    & 2                      & \textbf{10} \\ \hline
% % No. of trajectories           &                   &       &                        &      \\ \hline
% \multirow{4}{*}{Type of data} & 3D bounding boxes & yes   & yes                    & \textbf{yes}  \\
%                               & ego-car odometry  & yes   & no                     & \textbf{yes}  \\
%                               & point clouds      & yes   & no                     & \textbf{yes}  \\
%                               & 360$^\circ$ coverage      & no    & yes                    & \textbf{yes}  \\ 
%                               & intentional goal      & no    & no                     & \textbf{yes}  \\ \hline
                              
% \end{tabular}
% \end{center}
% \vspace{0.1cm}
% \caption{Comparison of driving scene datasets (KITTI, TrafficPredict, and ours) for future trajectory forecast. The total number of scenarios, number of frames, number of trajectories and type of data.}
% \label{tbl:dataset}\vspace{-0.6cm}
% \end{table}
%
% \begin{table}[]
%     \begin{minipage}{.5\linewidth}
%     %   \caption{}
%       \centering
%         \begin{tabular}{lccc}
%             \hline
            
%                             &                  KT~\cite{Geiger2012CVPR} & TP~\cite{ma2019trafficpredict} & OURS \\ \hline \hline
%             Scenarios        & 50    & 103                    & \textbf{213}     \\ \hline
%             Frames ($\times10^3$)          & 13.1      & \textbf{90}                       & 59.4     \\ \hline %59470
%             Classes           & 8     & 5                      & \textbf{8}  \\ \hline 
%             Intersections      &      &                       & \textbf{213}  \\ \hline 
%             FPS               & 10    & 2                      & \textbf{10} \\ \hline
%             % No. of trajectories           &                   &       &                        &      \\ \hline
%         \end{tabular}
%     \end{minipage}%
%     \begin{minipage}{.4\linewidth}
%       \centering
%         % \caption{comparison of types of data available}
%         \begin{tabular}{lccc}
%             \hline
%             Data &                  KT~\cite{Geiger2012CVPR} & TP~\cite{ma2019trafficpredict} & OURS \\ \hline \hline
%          3D Boxes & \checkmark   & \checkmark                    & \Checkmark  \\\hline
%         %   &&&&\\
%                               Odometry  & \checkmark   &                      & \Checkmark  \\\hline
%                               Point-cloud      & \checkmark   &                      & \Checkmark  \\\hline
%                               360$^\circ$ coverage      &     & \checkmark                    & \Checkmark  \\ \hline
%                               Intention-goal   &     &                      & \Checkmark  \\ \hline
%         \end{tabular}
%     \end{minipage} 
%     \caption{Comparison of driving scene datasets (KT:KITTI~\cite{Geiger2012CVPR}, TP:TrafficPredict~\cite{ma2019trafficpredict}, and our intersection dataset) 
% for future trajectory forecast. Our dataset contains larger number of scenarios, object classes, intersections, and sampling fequency with more descriptive information.}
% \label{tbl:dataset}\vspace{-0.6cm}
% \end{table}

%% full-size
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[]%\footnotesize
% \caption{Comparison of our dataset with driving scene datasets -- KITTI~\cite{Geiger2012CVPR} and TrafficPredict\cite{ma2019trafficpredict} -- for future trajectory forecast. %Our dataset contains larger number of scenarios, object classes, intersections, and sampling fequency with more descriptive information.
% }
% \begin{center}
% \begin{tabular}{llcccl}
% \hline
%                               &                   & KITTI & TrafficPredict & Ours \\ \hline \hline
% No. of scenarios              &                   & 50    & 103                    & \textbf{213}     \\ \hline
% No. of frames ($\times10^3$)                 &                   & 13.1      & \textbf{90}                       & 59.4     \\ \hline %59470
% No. of object classes                &                   & 8     & 5                      & \textbf{8}  \\ \hline 
% No. of intersections          &                   &      &                       & \textbf{213}  \\ \hline 
% Sampling frequency (fps)      &                   & 10    & 2                      & \textbf{10} \\ \hline
% % No. of trajectories           &                   &       &                        &      \\ \hline
% \multirow{6.5}{*}{Type of labels} & 3D bounding boxes & \checkmark   & \checkmark                    & \Checkmark  \\
%                               & Ego-car odometry  & \checkmark   &                      & \Checkmark  \\
%                               & LiDAR point cloud      & \checkmark   &                      & \Checkmark  \\
%                               & 360$^\circ$ coverage      & \checkmark    &                     & \Checkmark  \\ 
%                               & Intentional goal       &     &                      & \Checkmark  \\
%                               & Drivable area mask       &     &                      & \Checkmark  \\ \hline
% \end{tabular}
% \end{center}
% % \vspace{0.1cm}
% \label{tbl:dataset}%\vspace{-0.7cm}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Intersection Dataset}
% %
% A large dataset is collected in 4 urban areas in the San Francisco Bay Area. 
% %
% [[To rewrite]] This dataset includes scenarios from the Honda Research Institute 3D Dataset (H3D)~\cite{patil2019h3d} and additional scenarios annotated similarly as those in~\cite{patil2019h3d}. 
% %
% About 200 highly interactive scenes at complex intersections are chosen. 
% %
% It consists of LiDAR-based point clouds, 3D bounding boxes of traffic participants (8 classes including cars and pedestrians), odometry of the ego-car, and the corresponding 'zone' for each traffic participant. 
% %
% A comparison of KITTI, TrafficPredict and our dataset is shown in Table~\ref{tbl:dataset}.

% %%

% The point cloud data is acquired using a Velodyne HDL-64E S3 sensor and point cloud distortion correction is performed using the high-frequency GPS data. 
% %
% As highlighted in~\cite{patil2019h3d}, the 3D bounding boxes are labelled manually at 2Hz and linearly propagated to generate data at 10Hz. 
% %
% It comprises of the traffic participant's track-ID, 3D position (m), dimensions (m) and heading angle (rad). Odometry of the ego-car is obtained via Normal Distributive Transform (NDT)-based point cloud registration. 
% %
% The registered point cloud data is used to generate 5 intersection zones which are labelled from 0 through 4 in a clockwise direction, with 0 being the 'middle' zone~\ref{fig:main}. 
% %
% These spatial attributes are assigned to each traffic participant (forming its "intention category"). 
% %
% The dataset is available at http://usa.honda-ri.com/h3ds/
% %


\begin{table*}[!t]
\centering%\vspace{-0.6cm}
  \caption{Comparison of our new dataset with the driving datasets for trajectory prediction - KITTI~\cite{Geiger2012CVPR}, Apolloscape~\cite{ma2019trafficpredict}, and Argoverse~\cite{chang2019argoverse}. 
  }\label{tbl:dataset}%\vspace{-0.2cm}
\begin{tabular}{llcccc}
\hline
 & & KITTI~\cite{Geiger2012CVPR}~&~Apolloscape~\cite{ma2019trafficpredict}~&~Argoverse~\cite{chang2019argoverse}~&~Ours \\ \hline \hline
\multicolumn{2}{l}{No. of scenarios} & 50 & 103 &- & \textbf{213}     \\ \hline
\multicolumn{2}{l}{No. of frames ($\times10^3$)} & 13.1 & {90} &\textbf{192} &59.4     \\ \hline %59470
\multicolumn{2}{l}{No. of object classes} & 8 & 5& \textbf{15}&{8}  \\ \hline 
\multicolumn{2}{l}{Sampling frequency (fps)} & 10  & 2  & 10&\textbf{10} \\ \hline
\multicolumn{2}{l}{Trajectory duration ($sec$)}& flexible &  flexible & fixed (5)&\textbf{ flexible}  \\ \hline 
\multicolumn{2}{l}{No. of intersections}&- &  -&-&\textbf{255}  \\ \hline 
\multirow{6.5}{*}{\makecell{Type of~~~\\ ~labels}} 
& 3D bounding boxes & \checkmark&no &no & \Checkmark  \\
& Ego-car odometry  & \checkmark& no&no & \Checkmark  \\
& LiDAR point cloud & \checkmark&no &\checkmark & \Checkmark  \\
& 360$^\circ$ coverage& \checkmark &no&\checkmark& \Checkmark  \\ 
& Drivable area mask& no&no&\checkmark& \Checkmark \\
& Intentional goal  &no &no&no& \Checkmark  \\
\hline
                              
\end{tabular}%\vspace{-0.5cm}
\end{table*}





A large-scale dataset is collected in the San Francisco Bay Area (San Fransisco, Mountain View, San Mateo, and Santa Cruz), focusing on highly interactive scenarios at four-way intersections. We chose 213 scenarios in both urban and residential areas, which contain interactions between road users toward an environment. Our intersection dataset consists of LiDAR-based point clouds (full 360$^\circ$ coverage), track-IDs of traffic participants, their 3D bounding boxes, object classes (8 categories including cars and pedestrians), odometry of the ego-car, heading angle (in $rad$), drivable area mask, and potential destination as zone (intentional goal). \textcolor{red}{Fig.~\ref{fig:data1}} displays an example of the intersection, and top-down view maps generated from each scenario are visualized in \textcolor{red}{Fig.~\ref{fig:data2}-\ref{fig:data5}}. Also, we compare our dataset with other datasets~\cite{Geiger2012CVPR, ma2019trafficpredict, chang2019argoverse} in Table~\ref{tbl:dataset}.



%%
The point cloud data is acquired using a Velodyne HDL-64E S3 sensor, and distortion correction is performed using the high-frequency GPS data. Odometry of the ego-car is obtained via NDT-based point cloud registration. The labels are manually annotated at 2Hz and linearly interpolated to generate labels at 10Hz. %, similar to those of H3D dataset~\cite{patil2019h3d}. 
For zones, we use the registered point cloud data and divide the intersection by 5 regions which are labeled from 0 through 4 in a clockwise direction as illustrated in Fig.~\ref{fig:main}. Our new dataset will be released to the public.

